On First-Order Model-Based Reasoning

Reasoning semantically in first-order logic is notoriously a challenge. This paper surveys a selection of semantically-guided or model-based methods that aim at meeting aspects of this challenge. For first-order logic we touch upon resolution-based methods, tableaux-based methods, DPLL-inspired methods, and we give a preview of a new method called SGGS, for Semantically-Guided Goal-Sensitive reasoning. For first-order theories we highlight hierarchical and locality-based methods, concluding with the recent Model-Constructing satisfiability calculus.

==> mbr-fol-lift.tex <==
\subsection{The Model Evolution Calculus}

The practical success of DPLL-based SAT solvers suggested the goal
of lifting features of DPLL to the first-order level.
Research focused on {\em splitting first-order clauses},
seen as a way to improve the capability to handle non-Horn clauses.
Breaking first-order clauses apart is not as simple as in propositional logic,
because a clause stands for all its ground instances,
and literals share variables that are implicitly universally quantified.
Decomposing disjunction is a native feature in tableaux
(cf. the $\beta$-rule of semantic tableaux),
whose downside is represented by rigid variables,
as already discussed in Section~\ref{subsect:hypertab},
where we saw how hypertableaux offer a possible answer.

The quest for ways to split efficiently clauses such as $A(x) \vee B(x)$ led to
the {\em model evolution} (${\cal M}{\cal E}$) calculus \cite{MEC:AI:2008}.
Splitting $A(x) \vee B(x)$ yields a branch with $A(x)$,
meaning $\forall x A(x)$, and one with $\neg A(c)$,
the Skolemized form of $\neg \forall x A(x) \equiv \exists x \neg A(x)$.
Splitting in this way has the disadvantage that the signature changes,
and Skolem constants, being new, do not unify with other non-variable terms.
${\cal M}{\cal E}$ maintains a {\em context} $\Lambda$,
which is a finite set of literals,
representing a Herbrand interpretation $I_{\Lambda}$,
seen as a candidate partial model of the input set of clauses $S$.
The literals in $\Lambda$ may contain {\em variables}
(implicitly universally quantified as in clauses)
and {\em parameters},
used instead of Skolem constants to replace existentially quantified variables
(cf. the $\delta$-rule in semantic tableaux).
In order to determine whether 
$I_{\Lambda}\models L$, for $L$ an atom in the Herbrand base of $S$,
one looks at the most specific literal in $\Lambda$ that subsumes $L$;
in case of a tie, $L$  is picked with positive sign.
Clauses are written in the form $\Lambda \vdash C$,
so that each clause carries the context with itself.
If $I_{\Lambda}$ is not a model of $S$,
the inference system unifies input clauses against $\Lambda$
to find instances that are not true in $I_{\Lambda}$:
these instances are subject to splitting,
to modify $\Lambda$ and repair $I_{\Lambda}$.
Otherwise, the system recognizes that $\Lambda$ cannot be fixed and
declares $S$ unsatisfiable.
As DPLL uses {\em depth-first search with backtracking},
${\cal M}{\cal E}$ uses depth-first search with backtracking and {\em iterative deepening}
on term depth, which however may skew the search towards big proofs with small term depth.
${\cal M}{\cal E}$ was extended to handle equality \cite{MEE:JSC:2012},
and combined with superposition \cite{MEC+SUP:CADE2009}.

